Rich Knowledge Sources Bring Complex Knowledge Conflicts: Recalibrating Models to Reflect Conflicting Evidence

Question answering models can use rich knowledge sources -- up to one hundred retrieved passages and parametric knowledge in the large-scale language model (LM). Prior work assumes information in such knowledge sources is consistent with each other, paying little attention to how models blend information stored in their LM parameters with that from retrieved evidence documents. In this paper, we simulate knowledge conflicts (i.e., where parametric knowledge suggests one answer and different passages suggest different answers) and examine model behaviors. We find retrieval performance heavily impacts which sources models rely on, and current models mostly rely on non-parametric knowledge in their best-performing settings. We discover a troubling trend that contradictions among knowledge sources affect model confidence only marginally. To address this issue, we present a new calibration study, where models are discouraged from presenting any single answer when presented with multiple conflicting answer candidates in retrieved evidences.

==> images/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{cornflowerblue}{RGB}{100,149,237}
\definecolor{darkorange}{RGB}{255,140,0}
\definecolor{dimgray85}{RGB}{85,85,85}
\definecolor{gainsboro229}{RGB}{229,229,229}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{whitesmoke}{RGB}{245,245,245}

\begin{groupplot}[group style={group size=4 by 1}]
\nextgroupplot[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.09,0.5)},
  anchor=west,
  draw=lightgray204,
  fill=gainsboro229
},
tick align=outside,
tick pos=left,
title={Perturb 25\%},
x grid style={white},
xlabel=\textcolor{dimgray85}{Perturb 25\%},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=dimgray85},
xtick={0,1,2},
xticklabels={random,top-ret.,top-att.},
y grid style={white},
ylabel=\textcolor{dimgray85}{Percentage of All Answers},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=dimgray85},
ytick={0,50,100,150},
yticklabels={0,20,40,60}
]
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:-0.25,0) rectangle (axis cs:0.25,75.4);
\addlegendimage{ybar,ybar legend,draw=none,fill=cornflowerblue,very thin}
\addlegendentry{Original}

\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:0.75,0) rectangle (axis cs:1.25,48.66);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:1.75,0) rectangle (axis cs:2.25,48);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:-0.25,75.4) rectangle (axis cs:0.25,91.75);
\addlegendimage{ybar,ybar legend,draw=none,fill=whitesmoke,very thin}
\addlegendentry{Others}

\draw[draw=none,fill=whitesmoke,very thin] (axis cs:0.75,48.66) rectangle (axis cs:1.25,68.85);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:1.75,48) rectangle (axis cs:2.25,70.29);
\draw[draw=none,fill=darkorange,very thin] (axis cs:-0.25,91.75) rectangle (axis cs:0.25,100);
\addlegendimage{ybar,ybar legend,draw=none,fill=darkorange,very thin}
\addlegendentry{Substitute}

\draw[draw=none,fill=darkorange,very thin] (axis cs:0.75,68.85) rectangle (axis cs:1.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:1.75,70.29) rectangle (axis cs:2.25,100);
\draw (axis cs:0,75.4) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{75.4};
\draw (axis cs:1,48.66) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{48.66};
\draw (axis cs:2,48) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{48.0};
\draw (axis cs:0,88.25) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{8.25};
\draw (axis cs:1,65.35) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{31.15};
\draw (axis cs:2,66.79) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{29.71};

\nextgroupplot[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204,
  fill=gainsboro229
},
tick align=outside,
tick pos=left,
title={Perturb 50\%},
x grid style={white},
xlabel=\textcolor{dimgray85}{Perturb 50\%},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=dimgray85},
xtick={0,1,2},
xticklabels={random,top-ret.,top-att.},
y grid style={white},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=dimgray85},
ytick={0,50,100,150},
yticklabels={0,20,40,60}
]
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:-0.25,0) rectangle (axis cs:0.25,53);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:0.75,0) rectangle (axis cs:1.25,24.87);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:1.75,0) rectangle (axis cs:2.25,23.67);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:-0.25,53) rectangle (axis cs:0.25,75);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:0.75,24.87) rectangle (axis cs:1.25,51.92);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:1.75,23.67) rectangle (axis cs:2.25,51.07);
\draw[draw=none,fill=darkorange,very thin] (axis cs:-0.25,75) rectangle (axis cs:0.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:0.75,51.92) rectangle (axis cs:1.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:1.75,51.07) rectangle (axis cs:2.25,100);
\draw (axis cs:0,53) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{53.0};
\draw (axis cs:1,24.87) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{24.87};
\draw (axis cs:2,23.67) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{23.67};
\draw (axis cs:0,71.5) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{25.00};
\draw (axis cs:1,48.42) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{48.08};
\draw (axis cs:2,47.57) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{48.93};

\nextgroupplot[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.91,0.5)},
  anchor=east,
  draw=lightgray204,
  fill=gainsboro229
},
tick align=outside,
tick pos=left,
title={Perturb 75\%},
x grid style={white},
xlabel=\textcolor{dimgray85}{Perturb 75\%},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=dimgray85},
xtick={0,1,2},
xticklabels={random,top-ret.,top-att.},
y grid style={white},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=dimgray85},
ytick={0,50,100,150},
yticklabels={0,20,40,60}
]
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:-0.25,0) rectangle (axis cs:0.25,26.61);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:0.75,0) rectangle (axis cs:1.25,14.57);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:1.75,0) rectangle (axis cs:2.25,10.34);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:-0.25,26.61) rectangle (axis cs:0.25,54.83);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:0.75,14.57) rectangle (axis cs:1.25,43.17);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:1.75,10.34) rectangle (axis cs:2.25,40.53);
\draw[draw=none,fill=darkorange,very thin] (axis cs:-0.25,54.83) rectangle (axis cs:0.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:0.75,43.17) rectangle (axis cs:1.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:1.75,40.53) rectangle (axis cs:2.25,100);
\draw (axis cs:0,26.61) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{26.61};
\draw (axis cs:1,14.57) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{14.57};
\draw (axis cs:2,10.34) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{10.34};
\draw (axis cs:0,51.33) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{45.17};
\draw (axis cs:1,39.67) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{56.83};
\draw (axis cs:2,37.03) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{59.47};

\nextgroupplot[
axis background/.style={fill=gainsboro229},
axis line style={white},
legend cell align={left},
legend columns=3,
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,0)},
  anchor=south east,
  draw=lightgray204,
  fill=gainsboro229
},
tick align=outside,
tick pos=left,
title={Perturb 100\%},
x grid style={white},
xlabel=\textcolor{dimgray85}{Perturb 100\%},
xmajorgrids,
xmin=-0.5, xmax=2.5,
xtick style={color=dimgray85},
xtick={0,1,2},
xticklabels={random,top-ret.,top-att.},
y grid style={white},
ymajorgrids,
ymin=0, ymax=105,
ytick style={color=dimgray85},
ytick={0,50,100,150},
yticklabels={0,20,40,60}
]
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:-0.25,0) rectangle (axis cs:0.25,2.56);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:0.75,0) rectangle (axis cs:1.25,2.56);
\draw[draw=none,fill=cornflowerblue,very thin] (axis cs:1.75,0) rectangle (axis cs:2.25,2.56);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:-0.25,2.56) rectangle (axis cs:0.25,34.64);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:0.75,2.56) rectangle (axis cs:1.25,34.64);
\draw[draw=none,fill=whitesmoke,very thin] (axis cs:1.75,2.56) rectangle (axis cs:2.25,34.64);
\draw[draw=none,fill=darkorange,very thin] (axis cs:-0.25,34.64) rectangle (axis cs:0.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:0.75,34.64) rectangle (axis cs:1.25,100);
\draw[draw=none,fill=darkorange,very thin] (axis cs:1.75,34.64) rectangle (axis cs:2.25,100);
\draw (axis cs:0,2.56) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{2.56};
\draw (axis cs:1,2.56) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{2.56};
\draw (axis cs:2,2.56) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{2.56};
\draw (axis cs:0,31.14) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{65.36};
\draw (axis cs:1,31.14) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{65.36};
\draw (axis cs:2,31.14) node[
  scale=0.5,
  anchor=base,
  text=black,
  rotate=0.0
]{65.36};
\end{groupplot}

\end{tikzpicture}


==> test.tex <==
% This file was created with tikzplotlib v0.10.1.


\input{A.tikz}
\includegraphics[width=7.5cm][A.tikz]
